CAN Coach: Vehicular Control through Human Cyber-Physical Systems

This work addresses whether a human-in-the-loop cyber-physical system (HCPS) can be effective in improving the longitudinal control of an individual vehicle in a traffic flow. We introduce the CAN Coach, which is a system that gives feedback to the human-in-the-loop using radar data (relative speed and position information to objects ahead) that is available on the controller area network (CAN). Using a cohort of six human subjects driving an instrumented vehicle, we compare the ability of the human-in-the-loop driver to achieve a constant time-gap control policy using only human-based visual perception to the car ahead, and by augmenting human perception with audible feedback from CAN sensor data. The addition of CAN-based feedback reduces the mean time-gap error by an average of 73%, and also improves the consistency of the human by reducing the standard deviation of the time-gap error by 53%. We remove human perception from the loop using a ghost mode in which the human-in-the-loop is coached to track a virtual vehicle on the road, rather than a physical one. The loss of visual perception of the vehicle ahead degrades the performance for most drivers, but by varying amounts. We show that human subjects can match the velocity of the lead vehicle ahead with and without CAN-based feedback, but velocity matching does not offer regulation of vehicle spacing. The viability of dynamic time-gap control is also demonstrated. We conclude that (1) it is possible to coach drivers to improve performance on driving tasks using CAN data, and (2) it is a true HCPS, since removing human perception from the control loop reduces performance at the given control objective.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> introduction-old.tex <==
% jonathan rewrote all of this on 10/26 starting at 3:58

The goal of Lagrangian control is to control a few particles within a flow in order to effect the overall flow. In the domain of transportation, this may be carried out by control of a few vehicles in the flow of traffic in order to achieve a control objective. Approaches of Lagrangian control could include either modification of a vehicle's velocity, or its position---or position and velocity. In order to effect certain kinds of traffic phenomena, it is necessary to be able to control not just the velocity of a vehicle (which might leave significant space that would encourage lane changing) but also control the spacing between the control (ego) vehicle and the lead vehicle in order to influence the velocities of the vehicles behind through normal driver behaviors. 

Research has been done to evaluate the idea of Lagrangian control of traffic with automated vehicles, demonstrating that vehicle automation can smooth traffic waves, even with relatively low penetration rates both in simulation~\cite{vinitsky2018lagrangian} and in full-scale experiments~\cite{stern2017dissipation}. These controllers dampen traffic waves through prescribed time-gap following, but they depend on advanced sensing and computation from the vehicles of tomorrow in order to close the loop with an accuracy and dependability that is on par with human-driven vehicles, with a requirement of something around 5\% or more of the vehicles to be control vehicles.

This raises a motivating question: can a human driver drive in a manner that dampens traffic waves, and thus accelerate the potential to adopt Lagrangian control by having the human perform some tasks that might otherwise require advanced sensors? If a human driver can be enabled to accurately follow commands that would enable Lagrangian control, then it may be possible to rapidly deploy technology in the vehicles of today that combines the advanced perception found in human drivers with advice from a supervisory controller that provides updated time-gap set points to carry out a control objective.

In this paper, we ask drivers to follow a vehicle (the lead vehicle) in their vehicle (the ego vehicle) in order to determine how to positively improve time-gap following through the use of a CAN Coach. This CAN Coach uses information from the CAN bus such as instantaneous velocity along with estimates of the relative position and velocity of the lead vehicle. These data were collected using only data from the CAN in the ego vehicle.\footnote{This work was conducted under IRB approval \#200343.} Drivers are asked to follow a lead vehicle with several different objectives, as well as to follow an imaginary vehicle (a ``ghost'' vehicle) by using the CAN Coach to follow a space-gap, but without the visual feedback to the human-in-the-loop from the lead vehicle. 

Our results show that with the CAN Coach, coached drivers can closely control the time-gap\jms{time-gap?} between the lead vehicle and the ego vehicle, i.e. space as a function of speed. The driving behavior with the CAN Coach is significantly improved compared to when drivers are instructed to use their own perception to achieve the same level of control. When following the ghost vehicle, the driver is more effective than when instructed, but not as effective as with the CAN Coach with a lead vehicle. %This suggests that CAN Coach is an HCPS, since remov.\Rahul{Looks some inadvertent typo occurred here}\Matt{I was in the midst of incorporating the text from Sprinkle with the rest below, when I had to drop it and move my focus elsewhere}

%Introducing CAN, and why its a great data source 
Modern vehicles have \textit{controller area networks} (CANs) that are in place to facilitate communication between \textit{electronic control units} (ECUs) on the vehicle~\cite{farsi1999overview}. CAN uses a multi-master data bus where all messages are multicast. On board a typical vehicle there are dozens of systems which use the CAN, featuring hundreds of sensors, that support everything in the vehicle from optimal engine function to climate control to driver safety. Year by year, more electronic features are added (e.g., adaptive cruise control, blind spot monitoring, lane keep assist). The amount of data produced on the CAN will continue to accelerate as vehicles become increasingly automated.

%The data that is multicast on the CAN bus provides information about the car, the driver, and the external environment. CAN messages are often sent in the order of hundreds of Hertz, and the thousands of data signals are typically a standard eight bytes in size. This means gigabytes of data per hour are sent on a vehicle's CAN bus. 

Considering the ubiquity of CAN technology and the holistic nature of the data it provides, there is substantial potential for finding insights about drivers under various levels of vehicle automation~\cite{fugiglando2018driving,wakita2006driver}. Moreover, considering the real-time nature of the CAN and the increased number of sensors reporting data on it, it is now possible to imagine CAN applications that augment safety, improve eco-driving, or adjust vehicle following behavior.

%here is where to talk about the HCPS
Since CAN data is available widely within today's vehicle fleet, these applications could scale broadly and at low cost. The demonstrable value of CAN data is already established in commercial aftermarket applications. Insurance companies offer discounts on rates in exchange for a relatively reduced set of data on a driver available through the \textit{on board diagnostics} (OBD-II) interface (a subset of the data available on the CAN) to characterize driver behavior and ultimately risk~\cite{eling2020impact}. Major vehicle manufacturers now collect data on their vehicles, and collaborate on CAN data research~\cite{bazilinskyy2018graded, bazilinskyy2019continuous,seppelt2007making,wu2016traffic,wang2019early}. Like the rapid introduction of mobility applications that were created during the transition from traditional cell phones to smartphones~\cite{wong2010cell}, we expect a similar transition to occur on vehicles using data available on the CAN bus. 

The goal of this work is to illustrate a Human-in-the-loop CPS (HCPS) that is effective in controlling the time-gap of an individual vehicle in traffic flow, using CAN data to provide unique feedback to the human-in-the-loop. Though there has been discussion of the potential of CAN data to support application development \cite{fugiglando2018driving}, there have not yet been studies published showing that real-time CAN feedback to a human driver is effective in controlling speed and spacing on the roadway.

%what did we do in this paper, the contributions

%In this work we present evidence showing an HCPS effective at controlling time-gap for an individual vehicle on the roadway. We explore the nature and limitations of the HCPS with four tests: velocity matching, constant \textit{time-gap} (i.e., the time separation between a lead vehicle's rear bumper and the ego vehicle's front bumper when the follower travels at a constant speed\cite{loulizi2019steady}), constant time-gap with a dynamic target set point (dynamic time-gap), and an 'ablation study' to test the hypothesis that the human-in-the-loop is integral to the performance of the HCPS.

%We introduce \textit{CAN Coach}, a system that provides real-time feedback to the driver based on sensor data already available on the CAN bus. The driver is enabled to achieve a control task with the aid of CAN Coach delivering extrasensory feedback to the driver. In this work, the CAN Coach improves the ability of a driver to match the velocity of a leading car\Matt{check this is true}, to maintain a constant time-gap, and maintain differing constant time-gaps when prompted. This is all done using only data from the CAN\footnote{This work was conducted under IRB approval \#200343}. The human-in-the-loop is shown to be integral to the performance of the CAN Coach system in the 'ablation study', called 'Ghost Mode'. In Ghost Mode, the driver is given CAN Coach feedback but the lead vehicle is an abstracted 'ghost' vehicle instead of a real vehicle on the physical roadway. This totally removes the human perception of the lead vehicle from affecting control.

%Drivers' performance on the control objective suffers in Ghost Mode compared to feedback from the real physical system because of the critical nature of the human cognition as a part of the human-in-the-loop cyber-physical system. The driver cannot leverage their ability to visually assess the roadway and intuitive understanding of driving dynamics to achieve the control objective. However, Ghost Mode performance is still favorable in comparison to no CAN Coach at all \Matt{still need the numbers here}. When a driver is just prompted to achieve a control objective while following a real vehicle, the performance is worse than Ghost Mode when 'following' a virtual vehicle. \Paul{Is this difference true for any control objective, or should specific control objectives be specified?}

%In Ghost Mode, the 'vehicle' being followed isn't bound by reality. Here is where the door opens to powerful possibility. Instead of just matching some arbitrary property such as velocity matching or specific time-gap, both of which are additionally informed by the driver's own senses, the driver can be guided to follow feedback from emergent traffic phenomena that are abstract and out of the realm of the driver's senses.

% In this simple control objective, we illustrate the potential to ``coach'' drivers using only data from the CAN.

\subsection{Contribution and Outline}

The contribution of this article is a demonstration of an HCPS that is effective in controlling an individual vehicle in a traffic flow. The CAN-based feedback system that is used (CAN Coach) enables drivers to achieve precise control tasks they could not otherwise achieve by giving extrasensory feedback informing adjustments of velocity and spacing. In other words, the CAN Coach can coach drivers to achieve superhuman driving tasks, and can enable a human-in-the-loop to drive in a manner that could dampen traffic waves. If successful, the application could scale widely given the low cost of the technology and the pervasive availability of the vehicle sensors; this would demonstrate the feasibility to deploy Lagrangian control techniques with the vehicle fleet of today.

%The 'Ghost Mode' of CAN Coach guides driver velocity and spacing according to an arbitrary virtual 'car'; results from Ghost Mode driving show that when the physical car is taken out of the 2-car system, and the drivers' human processing of the system is taken away, the performance at the control objective suffers. This supports the claim the the CAN Coach System is a true human-in-the-loop cyber-physical system. 
%The mean and standard deviation of the time-gap when following a real car is X.XX / X.XX for 2.25 s set point and X.XX / X.XX for 1.8 s set point, in comparison to X.XX / X.XX for 2.25 s set point and X.XX / X.XX for 1.8 s set point in Ghost Mode. \Dan{I like the idea but not execution. Some modest framing should take care of this.} We caution that the results presented here are from a limited study on six drivers, so the generalizablity across populations of drivers remains an open question. 

%This work showcases a human-in-the-loop cyber-physical system that is effective in controlling the time-space of an individual vehicle. Furthermore, the technology can scale since it is low-cost and leverages common vehicle technology.

%\Matt{this may need to be moved or cut, too much text for contribution} Despite the reduced performance in comparison to CAN Coach feedback, the driver performs better at matching variable time-gaps in Ghost Mode (just a virtual car) than when just verbally prompted to follow at a certain time-gap behind an actual car. In other words, the driver is better at the driving task when it is totally abstract and given CAN Coach feedback, than when left to their own devices. This result from the Ghost Mode opens the possibility for relating more abstract driving concepts to actionable feedback for a driver.

%A real-time feedback system, CAN Coach, is built to read CAN data and compute the error between the desired  time-gap and the current time-gap. A set of experiments are conducted to compare the time-gap distribution of a driver under \textit{i}) \textit{Normal Driving} with no coaching and no prompting; \textit{ii}) \textit{Instructed Driving} with a prompt to follow a two second time-gap but no coaching; and \textit{iii}) \textit{Coached Driving} with CAN Coach that provides real time feedback to assist the driver in achieving a two second time-gap. Compared to normal and instructed driving,  The mean time-gap error using CAN Coach is reduced from 0.39 s (Normal) and 0.09 s (Instructed) to 0.01 s. The standard deviation of time-gap error is also reduced using CAN Coach by 72\% (compared to Normal) and 68\% (compared to Instructed). 

%There is serious potential for applications controlling abstract emergent macro-scale traffic phenomena with Ghost Mode relating an abstract idea to drivers.

The remainder of this article is organized as follows. In Section~\ref{sec:related_work}, we discuss works informing the formation of CAN Coach. In Section~\ref{sec:can_coach_system_background}, we provide an overview of CAN data, the CAN messages used at run-time, the hardware platform, and the software platform. In Section~\ref{sec:methodology}, we describe the feedback design and the experimental design. Section~\ref{sec:results} describes CAN data validation, and results of the CAN Coach system experiments. Finally, Section~\ref{sec:conclusion} outlines the planned extensions from our work presented here.

